Causal Disentanglement for Robust Long-tail Medical Image Generation

Counterfactual medical image generation effectively addresses data scarcity and enhances the interpretability of medical images. However, due to the complex and diverse pathological features of medical images and the imbalanced class distribution in medical data, generating high-quality and diverse medical images from limited data is significantly challenging. Additionally, to fully leverage the information in limited data, such as anatomical structure information and generate more structurally stable medical images while avoiding distortion or inconsistency. In this paper, in order to enhance the clinical relevance of generated data and improve the interpretability of the model, we propose a novel medical image generation framework, which generates independent pathological and structural features based on causal disentanglement and utilizes text-guided modeling of pathological features to regulate the generation of counterfactual images. First, we achieve feature separation through causal disentanglement and analyze the interactions between features. Here, we introduce group supervision to ensure the independence of pathological and identity features. Second, we leverage a diffusion model guided by pathological findings to model pathological features, enabling the generation of diverse counterfactual images. Meanwhile, we enhance accuracy by leveraging a large language model to extract lesion severity and location from medical reports. Additionally, we improve the performance of the latent diffusion model on long-tailed categories through initial noise optimization.

==> images/ag3.tex <==
\begin{algorithm}[t]
\caption{Training Procedure for Causal Disentanglement and Counterfactual Generation}
\label{alg:overall}
\begin{algorithmic}[1]
\Require 
  Dataset $D$ with images $x$ and text reports $c_t$, learning rates $lr_1, lr_2$
\Ensure 
  Optimized parameters $\theta_{\mathcal{E}_{\text{VAE}}}, \theta_{\mathcal{D}_{\text{VAE}}}, \theta_{\mathcal{T}}, \theta_{\text{UNet}}, \theta_{\mathcal{E}_{\text{Text}}}$

\State \textbf{Stage 1: Train VAE and Transformer}
\State Initialize $\theta_{\mathcal{E}_{\text{VAE}}}, \theta_{\mathcal{D}_{\text{VAE}}}, \theta_{\mathcal{T}}$, optimizer $\mathcal{O}_1$ with $lr_1$
\For{each training step on $D$}
    \State $x_A, x_B \gets$ sample a pair of images from $D$ 
    \State $z_A = \{ z_A^{1:n-1}, z_A^n \} \gets \mathcal{E}_{\text{VAE}}(x_A; \theta_{\mathcal{E}_{\text{VAE}}})$
    \State $z_A = (z_A^{\text{str}}, z_A^{\text{patho}})$, $z_B = (z_B^{\text{str}}, z_B^{\text{patho}})$
    \State $f_A \gets \mathcal{T}(z_A)$, $f_B \gets \mathcal{T}(z_B)$
    \State $z'_A = (z_A^{\text{str}}, z_B^{\text{patho}})$, $z'_B = (z_B^{\text{str}}, z_A^{\text{patho}})$
    \State Decode: $x'_A = \mathcal{D}_{\text{VAE}}(z'_A)$, $x'_B = \mathcal{D}_{\text{VAE}}(z'_B)$
    \State Compute losses:
    \State $L_{\text{VAE}} = L_{\text{recon}} + \alpha L_{\text{KL}} + \beta L_{\text{cls}}$
    \State $L_{\text{id}} = \|\mathcal{E}_{\text{VGG}}(x_A) - \mathcal{E}_{\text{VGG}}(x'_A)\|^2 + \|\mathcal{E}_{\text{VGG}}(x_B) - \mathcal{E}_{\text{VGG}}(x'_B)\|^2$
    \State $L_{\text{PC}} = \|\mathcal{E}_{\text{CXR}}(x_A) - \mathcal{E}_{\text{CXR}}(x'_B)\|^2 + \|\mathcal{E}_{\text{CXR}}(x_B) - \mathcal{E}_{\text{CXR}}(x'_A)\|^2$
    \State $L_{\text{total}} = L_{\text{VAE}} + \gamma L_{\text{id}} + \delta L_{\text{PC}}$
    \State Update parameters using $\mathcal{O}_1$
\EndFor

\State \textbf{Stage 2: Train Latent Diffusion Model}
\State Initialize $\theta_{\text{UNet}}, \theta_{\mathcal{E}_{\text{Text}}}$, optimizer $\mathcal{O}_2$ with $lr_2$
\For{each training step on $D$}
    \State Sample $(x, c_t)$, encode as $z = (z^{\text{str}},z^{\text{patho}})$
    \State Sample timestep $t$ and noise $\epsilon \sim \mathcal{N}(0,I)$
    \State Apply noise: $z^{\text{patho}}_{T} \gets \text{add\_noise}(z^{\text{patho}}, t, \epsilon)$
    \State Encode text: $e_t \gets \mathcal{E}_{\text{Text}}(c_t)$
    \State Predict noise: $\epsilon_{\text{pred}} \gets \text{UNet}(z^{\text{patho}}_{T}, t, e_t)$
    \State Compute loss: $L_{G} = \|\epsilon - \epsilon_{\text{pred}}\|^2$
    \State Update $\theta_{\text{UNet}}$ using $\mathcal{O}_2$
\EndFor

\State \textbf{return} $\theta_{\mathcal{E}_{\text{VAE}}}, \theta_{\mathcal{D}_{\text{VAE}}}, \theta_{\mathcal{T}}, \theta_{\text{UNet}}, \theta_{\mathcal{E}_{\text{Text}}}$
\end{algorithmic}
\end{algorithm}


==> sec/1_intro.tex <==
\section{Introduction}
\begin{comment}
\IEEEPARstart{W}{ith} the success of deep learning in medical image analysis, the performance of models has become increasingly dependent on large-scale, high-quality annotated datasets. However, the acquisition of medical data is often constrained by high costs and patient privacy concerns, leading to the scarcity of data for certain diseases and severe imbalance in data distribution across categories. This data imbalance not only limits the generalization capability of models but also affects their applicability in real-world scenarios. In recent years, with the rapid development of image generation techniques, generative models have been widely applied to alleviate the issues of insufficient medical data and imbalanced datasets, providing significant support for medical research and clinical practice.
\end{comment}

\IEEEPARstart{I}{n} recent years, deep learning technology has made significant advancements in the medical field, greatly improving the performance of medical image analysis tasks. However, challenges arise in model training due to issues such as privacy concerns, acquisition costs, and the scarcity of rare cases, leading to imbalanced data distribution. Specifically, in multi-label tasks like CXR (chest X-ray), models tend to favor common categories while overlooking long-tail categories. Although methods have been proposed to address the label imbalance problem in image recognition tasks, the results have been limited and lack generalizability. With the development of generative models, researchers have begun using image generation techniques to create synthetic data that can replace or supplement real medical images.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/img/moti0.png}
    \caption{Challenges of generative models in synthesizing medical images. a) Difficulty in learning complex pathological visual features under small-sample conditions, resulting in synthesized pathological features that are inaccurate or indistinct. b) Instability in the structure of synthesized medical images, severely compromising the reliability of the images. c) Overly strong structural control conditions applied to the images, reducing diversity and impairing the accuracy of pathological simulation.}
    \label{fig:enter-label}
\end{figure}

Early work on medical image synthesis primarily revolved around GANs (Generative Adversarial Networks) \cite{goodfellow2014generativeadversarialnetworks}. 
Compared to CNN (Convolutional Neural Network) methods\cite{ShwartzZiv2017OpeningTB}, GANs achieve the modeling of data distribution by focusing on the underlying probability density.
Therefore, GANs have been widely applied in tasks such as denoising\cite{Wang2018ConditionalGA}\cite{7934380}\cite{8340157}, reconstruction\cite{Yang2018DAGANDD}\cite{seitzer2018adversarialperceptualrefinementcompressed}\cite{Yu2017DeepDF}, and cross-modality image translation\cite{Zhao2018CraniomaxillofacialBS}\cite{Wolterink2017DeepMT}\cite{Cohen2018DistributionML}. 
However, the training of GANs involves unstable factors \cite{8253599}, which become particularly pronounced in few-shot tasks.
GANs struggle with generalizing from limited data, often leading to overfitting and mode collapse\cite{bau2019seeinggangenerate}. 
This problem is exacerbated when there is insufficient data to capture the full variability of the target distribution, resulting in poor synthesis performance and a lack of meaningful variation in generated samples. 
Consequently, GANs face significant challenges in generating high-quality, diverse images from limited samples in few-shot learning tasks.
Recently, diffusion models\cite{ho2020denoisingdiffusionprobabilisticmodels} have gradually entered the researchers' focus due to their ability to generate high-quality and diverse images. 
After pre-training, diffusion models can be fine-tuned to become powerful generators in specific domains.
To explore the potential of diffusion models in medical image synthesis tasks, researchers have conducted several studies on medical image synthesis and translation\cite{Chambon_2022}. 
The pre-trained text-conditioned LDM (Latent Diffusion Model)\cite{rombach2022highresolutionimagesynthesislatent} contains plenty of prior knowledge from natural language and can create synthetic medical image data by prompting relevant medical keywords or concepts of interest\cite{Chambon_2022}.
This approach offers an effective means for the realistic simulation of various pathological conditions. 
On the other hand, image translation methods based on diffusion models have the capability to generate high-quality images, providing assistance in alleviating the issue of modality loss.

However, diffusion models face the following limitations in medical image generation tasks:
\begin{itemize}
    \item \textbf{Sample Scarcity:} Due to the high costs, patient privacy concerns, and the inherent rarity of certain cases, medical image data suffers from scarcity and imbalance distribution. Diffusion models have difficulty in synthesizing images for rare concepts and long-tail categories. We need to consider how to improve their performance in few-shot tasks.
    \item \textbf{Low Precision:} Medical images carry complex pathological information, making it challenging for diffusion models to achieve precise and controllable pathological simulation. The pathological features in the generated images are often indistinct or inaccurate.Moreover, the structural instability of the synthesized images further affects their overall quality.
\end{itemize}

\subsection{Motivation}
To address these issues, we hope to develop a few-shot medical image generation method that enables precise and controllable pathology simulation on specified anatomical structures. As shown in the figure, this method leverages provided structural information and textual prompts to generalize pathological features across arbitrary lung structures. This approach holds remarkable value for clinical diagnosis and medical reference.Specifically, we need to address the following fundamental challenges:
\begin{itemize}
    \item How to enhance the generation quality for long-tail pathology categories and mitigate the few-shot issue. It is crucial to address the inaccuracy in the inference process caused by the low representation of long-tail category samples in the input space during the training of diffusion models.
    \item How to make the training process more focused on the precision of pathology simulation, ensuring that the generated pathological features are both accurate and clinically relevant.
    \item How to balance the guiding effects of structural information and text prompts. Excessive focus on structural information can reduce image diversity and the accuracy of pathological features.
\end{itemize}

In this paper, we propose a novel few-shot medical image generation method that achieves accurate and controllable pathological simulation by combining text prompts with structural information. Specifically, we utilize Stable Diffusion for text-to-image synthesis and incorporate ControlNet to introduce semantic masks as structural information, enhancing the structural stability of generated images. To further improve image diversity, we employ a mask ablation algorithm that randomly removes parts of the organ masks.
To enhance the accuracy of pathology simulation, we first re-annotate the report data using GPT-4o-mini. This process focuses the reports on key pathological details, such as location and severity of pathologies, while removing redundant information to improve alignment between reports and images (as shown in Fig.1). Additionally, we incorporate CausalVAE to disentangle pathological information through causal relationships, thereby enhancing the model's ability to learn pathological features.
Given that long-tail samples constitute only a small fraction of the input space during training, the model may treat these inputs as out-of-distribution during inference. To address this, we introduce the SeedSelect method, which selects seed regions from the noise space that are more likely to generate long-tail pathological images, effectively mitigating the few-shot challenge.

\subsection{Contribution}
In summary, our contributions are as follows:
\begin{itemize}
    \item We designed a few-shot medical image synthesis framework that enables diversified data generation under conditions of limited and imbalanced medical image data.
    \item We improved the accuracy of pathology simulation and the stability of the image structure by combining text guidance and structural information control.
    \item  We conducted detailed evaluations of the method in terms of visual quality and pathological features, validating the reliability of our approach.
\end{itemize}

The remainder of this article is organized as follows: Section 2 presents several related works. Section 3 provides the details of our approach. The corresponding experimental results and analysis are given in Section 4. Finally, we discuss the limitations and our future work and conclude this paper in Section 5.


==> sec/2_rework.tex <==
\section{Related Work}
\subsection{Few-shot Image Generation}
Few-shot image generation (FSIG) aims to generate diverse and high-quality images with minimal training data. Traditional methods typically fine-tune pre-trained generative models, but this method often leads to overfitting when data is limited. To address this, researchers have proposed methods like EWC, AdAM, and RICK, which retain important weights to avoid overfitting, along with regularization and data augmentation techniques (e.g., BSA and FreezeD) to improve generalization. In addition to improving discriminators, generative architectures like FastGAN have been proposed to avoid mode collapse in few-shot scenarios. However, these methods generally require substantial computational resources. Recent approaches, such as Textual Inversion (Gal et al., 2023a) and Dreambooth (Ruiz et al., 2023), generate instance-specific images using a few reference samples in pre-trained generative models, but they struggle with generating class concepts effectively and require long training times. Dvir Samuel et al. presented a new perspective on the few-shot problem, suggesting that when generating rare concepts, the diffusion model observes only a small part of the input space during training. This means that, during generation, the model may view many random inputs as out-of-distribution data, leading to generation failures. To address this issue, they proposed the SeedSelect method, which selects suitable generation seeds in the noise space to effectively improve the performance of diffusion models in few-shot tasks. 

\subsection{Diffusion Model Based Controllable Image Synthesis}
In recent years, diffusion models have garnered widespread attention in the field of image generation. Ho et al. first introduced Denoising Diffusion Probabilistic Models (DDPM), enabling high-quality image synthesis through a denoising process. To address the issues of high computational cost in pixel space and slow inference, Rombach et al. applied diffusion models to the latent space of a pre-trained VAE, proposing Stable Diffusion, which enables training on limited computational resources while retaining both quality and flexibility.

Text-guided methods focus on adjusting prompts or manipulating model features to influence the generated content. For instance, Prompt-to-Prompt enables fine-tuning of generated content through localized modifications to the prompts, while InstructPix2Pix incorporates natural language instructions to control the content and style of generated images, enhancing the model's responsiveness to user commands.

In order to add spatial  conditioning controls to diffusion models, MakeAScene leverages semantic segmentation maps to provide scene layout control, combining this with text prompts for more precise generation. MaskSketch uses unpaired masks and sketches as input to generate structured content. ControlNet introduces a flexible framework that incorporates zero-convolution modules into diffusion models, enabling integration of multiple conditional images (such as edge maps, depth maps, and skeleton poses) into the generation process while preserving the capabilities of the pretrained model. These approaches significantly enhance the flexibility and effectiveness of conditional control, enabling personalized and task-specific image generation.

\subsection{Medical Image Synthesis}
Medical image synthesis based on generative models has been proven to be an effective approach for medical data augmentation. Depending on the input conditioning modality, generative methods can be divided into image-to-image translation methods and text-to-image synthesis methods.

Image translation methods utilize source modality information to synthesize medical images in the same modality or a target modality. SynDiff introduced a method based on adversarial diffusion models, enabling bilateral translation between MRI and CT modalities. SegGuidedDiff employs diffusion models that incorporate multi-class anatomical segmentation masks at each sampling step to achieve anatomically controlled mask-to-image synthesis for breast MRI and abdominal/neck-to-pelvis CT, and it proposes a random mask ablation strategy to enhance diversity in image generation. FairDiff utilizes 3D point clouds with mask images to achieve boundary control and synthesize SLO fundus images, enhancing data fairness. These methods leverage specific structural information to synthesize images, compensating for missing modalities and enhancing data volume. However, there has been limited research on generating images with specified pathology.

By leveraging natural language priors, text-conditioned diffusion models can flexibly guide image synthesis using various forms of text input, such as labels or detailed reports. This kind of generative methods can directly construct text-image medical data pairs, providing a large amount of annotated data for medical applications. RoentGen explored the use of diffusion models to generate high-fidelity, diverse synthetic CXR images based on text prompts and validated its effectiveness for data augmentation. LLM-CXR leverages pretrained large language models' (LLM) existing question-answering and instruction-following capabilities to achieve both text generation from images and image generation from text. These methods show promising results in lesion simulation; however, they do not incorporate edge information, and the sampling from random noise results in unstable image structures, affecting image quality. EMIT-DIFF combines edge information of objects to guide the synthesis process, preserving the essential features of the original medical images and introducing enhanced text to guide the synthesis for data augmentation. However, the enhanced text only addresses image quality and organ information without including pathological details.



==> sec/3_method.tex <==
\section{Method}
\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{images/img/method1.png}
    \caption{1.}
    \label{fig:enter-label}
\end{figure*}
In this section, we detail our method. Fig. illustrates our framework, which includes four key components:1) text-image generation model; 2) ControlNet structural information control module; 3) seed optimization module; 4) causal disentangling module.

\subsection{Disease Representation(VAE)}
Variational Autoencoders (VAEs) can effectively learn representations of medical images. The encoder in a VAE maps these high-dimensional medical images into a lower-dimensional latent space $z$, which serves as a compressed representation capturing the essential features of the image, including disease characteristics and anatomical structures.
The objective of the VAE is to learn the distribution of the latent variables $z$ by optimizing the Evidence Lower Bound (ELBO), ensuring that the latent representations effectively describe the data and support generative tasks. The ELBO is defined as:
\[
\mathcal{L} = \mathbb{E}_{q_\phi(z|x)}[\log p_\theta(x|z)] - D_{KL}(q_\phi(z|x) \| p(z)),
\]
where $q_\phi(z|x)$ is the approximate posterior distribution predicted by the encoder, $p_\theta(x|z)$ is the likelihood distribution predicted by the decoder, and $D_{KL}$ represents the Kullback-Leibler divergence between the approximate posterior $q_\phi(z|x)$ and the prior $p(z)$.
The latent representation $z$ learned by the encoder captures critical pathological features. These features can be leveraged for classification, segmentation and generative tasks.
\subsection{Generation Module}
\subsubsection{Denoising Diffusion Probabilistic Model}
The Denoising Diffusion Probabilistic Model (DDPM)\cite{ho2020denoisingdiffusionprobabilisticmodels} is a latent variable model for generation.
In the defined forward diffusion process $q(x_t|x_{t-1})$, given data $x_0\in\mathbb{R}^n$ is gradually perturbed by adding Gaussian noise in steps. This process can be defined as:
\begin{equation}q(\mathbf{x}_t|\mathbf{x}_{t-1})=\mathcal{N}(\mathbf{x}_t;\sqrt{1-\beta_t}\mathbf{x}_{t-1},\beta_t\mathbf{I})\end{equation}
where $\beta_t\in(0,1)$ represents the variance schedule across diffusion steps, and $x_{t}$
denotes the intermediate state image at step $t$.
In the reverse process, the task is to progressively denoise each step’s perturbation, gradually restoring the original data distribution. 
\begin{equation}p_\theta(x_{t-1}|x_t)=\mathcal{N}(x_{t-1};\mu_\theta(x_t,t),\sigma_t^2I)\end{equation}
where $\theta$ represents the model parameters. To achieve a simpler and more stable training framework, Ho et al. proposed training a model 
$\epsilon_\theta(x_t,t)$ to predict the noise 
$\epsilon$ instead of directly parameterizing $\mu_\theta(x_t,t)$ as a neural network. By reparameterization, the objective function is simplified as follows:
\begin{equation}L_\mathrm{simple}=\mathbb{E}_{t,\mathbf{x}_0,\boldsymbol{\epsilon}}\left[\|\boldsymbol{\epsilon}-\boldsymbol{\epsilon}_\theta(\mathbf{x}_t,t)\|^2\right]\end{equation}

\subsubsection{Seed Optimization Module}
In the task of few-shot medical image generation, we utilize a small set of real medical images from long-tail categories ($I_1, I_2, \dots, I_k$) to optimize the initial noise input $Z^T$, enabling the generation of images that better align with pathological features.

Pathological semantic consistency measures the semantic similarity between the generated medical image $I_G$ and the reference images $I_1, \dots, I_k$. 
The reference medical images are encoded using pre-trained CXR-CLIP image encoder to obtain pathological feature vectors $f_1, \dots, f_k$, and their centroid (mean vector) is computed as: $\mu_v = \text{mean}(f_1, \dots, f_k)$.
The generated medical image is also encoded to obtain its feature vector $f_G$. The pathological semantic loss is defined as:
\begin{equation}
L_{\text{P}} = \text{dist}_v(\mu_f, f_G),
\end{equation}
where $\text{dist}_f$ represents the Euclidean distance between the centroid $\mu_f$ and the feature vector $f_G$. This loss ensures that the generated medical image accurately reflects the pathological features present in the reference images.

Anatomical structure consistency measures the similarity between the latent representation $z_G^0$ of the generated medical image and the encoded representations of the reference images.The encoder $E$ of pre-trained VAE is used to encode the reference medical images $I_1, \dots, I_k$, resulting in the latent representations $z_1, \dots, z_k$.
The anatomical structure loss is defined as:
\begin{equation}
L_{\text{A}} = \frac{1}{k} \sum_{i=1}^k \text{dist}_z(z_i, z_G^0),
\end{equation}
where $\text{dist}_z$ represents the mean squared error (MSE) loss at the pixel level. This loss ensures that the anatomical structure of the generated image is consistent with the reference medical images. 

The combined requirements of pathological semantics and anatomical structure consistency are captured in the final loss defined as:
\begin{equation}
L_{\text{Seed}} = \lambda L_{\text{P}} + (1 - \lambda) L_{\text{A}},
\end{equation}
where the hyperparameter $\lambda$ controls the trade-off between semantic consistency and anatomical structure consistency.During the optimization process, $z_G^T$ is updated by backpropagating the total loss $L_{\text{Seed}}$. This approach does not modify the parameters of the pre-trained diffusion model, ensuring computational efficiency and model stability.

\subsubsection{ControlNet Module}
ControlNet is a neural network architecture that enables pretrained models to incorporate spatial conditional control through spatially localized, task-specific images. 

ControlNet incorporates additional conditional inputs $c$ into pretrained models by freezing the original model's parameters $\Theta$ and creating a trainable copy with parameters $\Theta_{c}$. This design allows the model to retain its original capabilities while learning to adapt to new conditions. The basic computation of ControlNet is as follows:
\begin{equation}
y_c = F(x; \Theta) + Z(F(x + Z(c; \Theta_{z1}); \Theta_c); \Theta_{z2})
\end{equation}
where $F(x; \Theta)$ represents the output of the original model,  
$Z(\cdot; \cdot)$ is a zero convolution layer,  
$c$ is the input conditional control signal (e.g., semantic segmentation mask). The initialization of the zero convolution layers $Z(\cdot)$ ensures that no random noise is introduced into the model at the beginning of training.
Therefore, the initial output $y_c$ equals the original output $y$:
\begin{equation}
y_c = y = F(x; \Theta).
\end{equation}
With this design, ControlNet can gradually learn the influence of the conditional input on the generation during the training process.
\subsection{Counterfactual Diversity Generation Module(CausalVAE)}
Medical image representations are often highly coupled, meaning that different tissues, lesions, and background information in the image are encoded within the same feature space. This makes the relationships between them complex and interdependent, which makes it difficult for the model to distinguish the independent effects of each component, thereby reducing the interpretability of the image representation.

\subsection{Training Strategies}
When introducing semantic masks to control the structural stability of synthesized images, we encountered the following issues. 

(1) When the constraints are too strong, the synthesized images strictly adhere to the structural information, making it difficult to accurately simulate pathologies that cause structural changes in the lungs or heart. 

(2) Although we used relatively loose structural information during training, the masks inevitably carry certain pathological information, which can mislead the model in terms of the original structural layout. 

In summary, the model's control over structural information requires  flexibility to ensure accurate simulation of visual features. 
It is necessary to balance between mask fidelity and the effectiveness of text guidance.

In SegGuidedDiff, the model demonstrates high fidelity to the mask.
To address the partial label problem caused by incomplete annotation in the mask, a random mask ablation strategy was designed to train the model to fill in or infer missing structural information and enhance the model's generalization and flexibility.
We adopted SegGuidedDiff's training strategy by using semantic masks in which the annotated organs include three categories: left lung, right lung, and heart. 
In half of the training steps, we randomly ablated one or two of these categories in the semantic masks to construct a dataset with partially missing labels. This training approach improves the model's flexibility in handling image layouts.


==> tables/AUC.tex <==
\begin{table*}[h!]
\centering
\caption{AUROC}
\label{tab:auc}
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Metric} & \textbf{Atel.} & \textbf{Cnsl.} & \textbf{Pmtx.} & \textbf{Edema} & \textbf{Eff.} & \textbf{Pna.} & \textbf{Cmgl.} & \textbf{Les.} & \textbf{Frac.} & \textbf{Opac.} & \textbf{ECm.} & \textbf{Avg.} \\
\midrule
RoentGen & 0.7408 & 0.7821 & 0.7256 & 0.6942 & \textbf{0.8155} & 0.5933 & 0.7324 & 0.6157 & 0.5926 & 0.7318 & 0.7848 & 0.7099 \\
UniXGen  & 0.7822 & 0.7359 & 0.6507 & 0.7718 & 0.7360 & 0.7024 & \textbf{0.8068} & 0.7056 & 0.6979 & 0.7710 & 0.8035 & 0.7422 \\
LLM-CXR  & 0.7893 & 0.8098 & 0.7389 & 0.7949 & 0.7992 & 0.7467 & 0.7689 & 0.7695 & 0.7244 & \textbf{0.8545} & 0.8168 & 0.7830 \\
\hline
Ours     & \textbf{0.8556} & \textbf{0.8304} & \textbf{0.7868} & \textbf{0.8089} & 0.8125 & \textbf{0.8012} & 0.7748 & \textbf{0.8375} & \textbf{0.7416} & 0.8473 & \textbf{0.8196} & \textbf{0.8106} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/F1.tex <==
\begin{table*}[h!]
\centering
\caption{F1 Score}
\label{tab:f1}
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Metric} & \textbf{Atel.} & \textbf{Cnsl.} & \textbf{Pmtx.} & \textbf{Edema} & \textbf{Eff.} & \textbf{Pna.} & \textbf{Cmgl.} & \textbf{Les.} & \textbf{Frac.} & \textbf{Opac.} & \textbf{ECm.} & \textbf{Avg.} \\
\hline
RoentGen & 0.7860 & 0.7067 & 0.6897 & 0.6266 & 0.7390 & 0.4681 & 0.7410 & 0.5616 & 0.6963 & 0.7248 & 0.6924 & 0.6757 \\
UniXGen  & 0.8398 & 0.6996 & 0.5231 & 0.7587 & 0.6868 & 0.6397 & 0.7340 & 0.5438 & 0.6231 & 0.7560 & 0.7519 & 0.6870 \\
LLM-CXR  & 0.8313 & 0.7835 & 0.6813 & \textbf{0.7819} & 0.7937 & 0.7304 & \textbf{0.8151} & 0.7447 & 0.6921 & \textbf{0.8392} & 0.7826 & 0.7702 \\
\hline
Ours     & \textbf{0.8591} & \textbf{0.8103} & \textbf{0.8028} & 0.7801 & \textbf{0.8174} & \textbf{0.7825} & 0.8018 & \textbf{0.7581} & \textbf{0.7857} & 0.8271 & \textbf{0.7947} & \textbf{0.8019} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/Trans.tex <==
\begin{table}[htbp]
    \centering
    \caption{Impact of Transformer Layers \( k \) on Image Generation Performance (Training for 10k Steps)}
    \label{tab:transformer_layers}
    \begin{tabular}{cccc}
        \toprule
        \textbf{Transformer Layers} \( k \) & \textbf{FID} & \textbf{mAUC} & \textbf{Training Time} \\
        \midrule
        0  & 8.2486 & 0.7184  & 6h35min \\
        6  & 7.2781 & 0.7551  & 7h47min \\
        12 & 7.2774 & 0.8104  & 8h15min \\
        18 & 7.2689 & 0.8160  & 9h46min \\
        24 & 7.2670 & 0.8171  & 10h39min \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/dis.tex <==
\begin{table}[htbp]
    \centering
    \caption{Impact of Disentangled Vector Count \( n \) on Image Generation Performance (Training for 10k Steps)}
    \label{tab:disentangled_vectors}
    \begin{tabular}{crc}
        \toprule
        \textbf{Disentangled Vectors} \( n \) & \textbf{FID} & \textbf{mAUC} \\
        \midrule
           5 & 6.9121 & 0.7583  \\
           6 & 6.8164 & 0.7926 \\
           7 & 7.2689 & 0.8106 \\
           8 & 7.2646 & 0.8154 \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/downstream2.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of Localization Results}
\label{tab:comparison}
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{\textbf{T(IoU)}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Disease Categories}} & \multirow{2}{*}{\textbf{Mean}} \\
\cmidrule(lr){3-7}
& & \textbf{Atelectasis} & \textbf{Cardiomegaly} & \textbf{Effusion} & \textbf{Pneumonia} & \textbf{Pneumothorax} & \\
\midrule
\multirow{5}{*}{0.1} 
& ResNet18 & 0.59 ± 0.00 & 0.81 ± 0.02 & 0.73 ± 0.00 & 0.23 ± 0.00 & 0.38 ± 0.01 & 0.55 ± 0.01 \\
& ResNet18 (SD) & 0.39 ± 0.03 & 0.90 ± 0.02 & 0.65 ± 0.01 & 0.30 ± 0.04 & 0.39 ± 0.05 & 0.53 ± 0.03 \\
& ResNet18 (SD+VAE) & 0.58 ± 0.01 & 0.91 ± 0.04 & 0.65 ± 0.01 & 0.79 ± 0.01 & 0.28 ± 0.01 & 0.64 ± 0.02 \\
& ResNet18 (Ours) & 0.64 ± 0.01 & \textbf{0.99 ± 0.02} & 0.66 ± 0.01 & 0.73 ± 0.02 & 0.29 ± 0.02 & 0.66 ± 0.02 \\
\midrule
\multirow{5}{*}{0.3} 
& ResNet18 & 0.24 ± 0.00 & 0.46 ± 0.01 & 0.30 ± 0.00 & 0.17 ± 0.00 & 0.13 ± 0.00 & 0.26 ± 0.00 \\
& ResNet18 (SD) & 0.29 ± 0.01 & 0.55 ± 0.02 & 0.31 ± 0.01 & 0.22 ± 0.00 & 0.22 ± 0.00 & 0.30 ± 0.00 \\
& ResNet18 (SD+VAE) & 0.20 ± 0.00 & 0.45 ± 0.01 & 0.19 ± 0.00 & 0.02 ± 0.00 & 0.00 ± 0.00 & 0.26 ± 0.01 \\
& ResNet18 (Ours) & 0.20 ± 0.01 & 0.48 ± 0.02 & 0.40 ± 0.02 & \textbf{0.46 ± 0.02} & 0.20 ± 0.00 & 0.33 ± 0.02 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/ds2.tex <==
\begin{table}[ht]
\centering
\caption{Comparison of Lesion Localization Results}
\label{tab:LL}
\begin{tabular}{cccccc}
\toprule
\textbf{Category} & \textbf{Model} & \textbf{T(IoU) = 0.1} & \textbf{T(IoU) = 0.3} \\
\midrule
\multirow{4}{*}{Atelectasis} 
    & Chestx-ray8 & 0.53 ± 0.02 & 0.25 ± 0.01 \\
    & AGXNet      & \textbf{0.64 ± 0.03} & 0.22 ± 0.02 \\
    & MBR(Ours)   & 0.63 ± 0.02 & \textbf{0.29 ± 0.01} \\
\midrule
\multirow{4}{*}{Cardiomegaly} 
    & Chestx-ray8   & 0.77 ± 0.03 & 0.47 ± 0.02 \\
    & AGXNet     & \textbf{0.93 ± 0.03} & 0.54 ± 0.02 \\
    & MBR (Ours)   & 0.85 ± 0.02 & \textbf{0.63 ± 0.02} \\
\midrule
\multirow{4}{*}{Effusion} 
    & Chestx-ray8    & 0.72 ± 0.01 & 0.31 ± 0.01 \\
    & AGXNet     & 0.66 ± 0.02 & 0.38 ± 0.01 \\
    & MBR (Ours)   & \textbf{0.75 ± 0.02} & \textbf{0.41 ± 0.02} \\
\midrule
\multirow{4}{*}{Pneumonia} 
    & Chestx-ray8          & 0.31 ± 0.18 & 0.17 ± 0.01 \\
    & AGXNet     & 0.70 ± 0.04 & \textbf{0.45 ± 0.01} \\
    & MBR (Ours)   & \textbf{0.72 ± 0.03} & 0.39 ± 0.02 \\
\midrule
\multirow{4}{*}{Pneumothorax} 
    & Chestx-ray8    & 0.38 ± 0.02 & 0.14 ± 0.01 \\
    & AGXNet     & 0.34 ± 0.06 & 0.20 ± 0.01 \\
    & MBR (Ours)   &\textbf{ 0.38 ± 0.01} & \textbf{0.21 ± 0.01} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/sota.tex <==
\begin{table*}[ht]
\centering
\caption{Comparison of text-to-image generation performance on the MIMIC-CXR and the OpenI datasets.}
\begin{tabular}{ccccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c}{\textbf{MIMIC-CXR}} & \multicolumn{5}{c}{\textbf{OpenI}} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-11}
                 & \textbf{FID\cite{FID}↓} & \textbf{NIQE\cite{NIQE}↓} & \textbf{MS-SSIM\cite{ms}↑} & \textbf{IS\cite{IS}↑} & \textbf{PSNR\cite{psnr}↑} & \textbf{FID↓} & \textbf{NIQE↓} & \textbf{MS-SSIM↑} & \textbf{IS↑} & \textbf{PSNR↑} \\ \hline
Stable Diffusion & 14.5194        & 5.7455         & 1             & 2        &          & 11.3305 & 5.7455  &               &         &          \\
RoentGen         &           &           &               &         &          &           &           &               &         &          \\
UniXGen          &           &           &               &         &          &           &           &               &         &          \\
LLM-CXR          &           &           &               &         &          &           &           &               &         &          \\ \hline
Ours             &           &           &               &         &          &           &           &               &         &          \\ \hline
\end{tabular}
\label{tab:my-table}
\end{table*}


